SLR-Eval: Benchmarking LLM Agents on Real-World Software Specification Design

As software engineering (SWE) agents grow more proficient at coding, the bottleneck is shifting from implementation to designing specifications. However, existing coding benchmarks primarily evaluate implementation-level reasoning: whether an agent can write code that satisfies a given specification. We argue that the next frontier for SWE agents is specification-level reasoning: the ability to design system specifications that are well defined, consistent, and effective. To evaluate this capability, we introduce SLR-Eval, a novel benchmark built from real Request for Comments (RFC) design proposals and maintainer reviews. SLR-Eval comprises 58 tasks and 1,726 human-verified rubric criteria across seven production open-source systems (Linux, Kubernetes, Rust, Python, React, vLLM, and TVM). Given an initial specification, the codebase, and past RFCs, the agent must identify deficiencies in the proposed specification and design revisions to resolve them. Across 23 frontier SWE agents, the best-performing agent achieves a score of only 0.447 out of 1, and 35.6% of expert-identified criteria are missed by every agent evaluated. We will open-source SLR-Eval and its dataset construction pipeline.

==> sections/07_limitations.tex <==
\section{Limitations}
\begin{itemize}
    \item Historical discussion is an incomplete reference for useful review. Accepted decisions are evidence-backed targets, not an exhaustive account of valid designs.
    \item Selection of eventually accepted, heavily discussed proposals limits coverage of rejected proposals and routine design work. Linux proposals may already include implementation material.
    \item Historical project snapshots approximate the information available to reviewers. Runtime cutoff controls do not remove potential exposure to public discussions during model training.
    \item Human validation uses graduate researchers, including benchmark authors where applicable, and covers 28 responses from three agents. Historical community discussion is not a matched human-performance baseline.
\end{itemize}

